Towards Pragmatic Semantic Image Synthesis for Urban Scenes

The need for large amounts of training and validation data is a huge concern in scaling AI algorithms for autonomous driving. Semantic Image Synthesis (SIS), or label-to-image translation, promises to address this issue by translating semantic layouts to images, providing a controllable generation of photorealistic data. However, they require a large amount of paired data, incurring extra costs. In this work, we present a new task: given a dataset with synthetic images and labels and a dataset with unlabeled real images, our goal is to learn a model that can generate images with the content of the input mask and the appearance of real images. This new task reframes the well-known unsupervised SIS task in a more practical setting, where we leverage cheaply available synthetic data from a driving simulator to learn how to generate photorealistic images of urban scenes. This stands in contrast to previous works, which assume that labels and images come from the same domain but are unpaired during training. We find that previous unsupervised works underperform on this task, as they do not handle distribution shifts between two different domains. To bypass these problems, we propose a novel framework with two main contributions. First, we leverage the synthetic image as a guide to the content of the generated image by penalizing the difference between their high-level features on a patch level. Second, in contrast to previous works which employ one discriminator that overfits the target domain semantic distribution, we employ a discriminator for the whole image and multiscale discriminators on the image patches. Extensive comparisons on the benchmarks GTA-V $\rightarrow$ Cityscapes and GTA-V $\rightarrow$ Mapillary show the superior performance of the proposed model against state-of-the-art on this task.

==> draft.tex <==
A recent work~\cite{splicingvit} has considered using ViT features for perceptual losses in style transfer. However, using ViT features is still under-explored and has not been yet materialized for I2I tasks. In this work, we show how we can leverage ViT to preserve content during translation.

 Most importantly, EPE~\cite{epe} uses a similar strategy but goes further by training the whole pipeline (generator + discriminator) on image crops to prevent the discriminator from overfitting on larger visual cues in the image. 

 The patch discriminator is a convolutional network that processes the image resulting in a  matrix of scores in $[0,1]$, denoting the realism of different patches in the image.

 %To train a model in an unpaired environment, where the model is presented mismatched images and labels in each iteration, they mostly employ paired datasets (like Cityscapes).


h%ave achieved remarkable results without needing access to paired data, they operate on ideal assumptions which reduce the applicability of these models in real-life. Mainly, they use paired datasets (like Cityscapes) to train a model in an unpaired setting, where the model is shown unaligned images and labels in each iteration. 

%that source domain (labels) and the target domain (images) share the same semantic distribution (class distribution). Specifically, they offer a less real

%These works train their models in an aligned fashion on a dataset containing human-annotated images collected in real life. We argue that such a setting would practically lead to supervised training. On the other hand, a truly unpaired setting would rather consist of 2 datasets (images and labels) with different class distributions. Two research questions thus naturally arise:\textit{ what would a realistic unpaired training scheme for SIS look like in autonomous driving applications? And how can cross-domain layout discrepancies be mitigated? }  

%To answer the first question, we propose a realistic unpaired training setup for SIS to facilitate its usage in autonomous driving applications. We use 2 sets for training: labels generated from graphics simulators and street-level images recorded in real life (Figure \ref{fig:teaser}). This setup melds the isolated advantages of synthetic-to-real image translation and unpaired SIS because it uses cheaply available synthetic data but offers more controllability as the input to the model is only a label map (not an image). 


%synthetic data can help scale AI perception algorithms by alleviating the need for expensive annotations. Compared to traditional graphics simulators, Generative Adversarial Networks (GANs) have the advantage of producing photorealistic images of urban scenes. In particular, conditional GANs (cGANs) can translate semantic layouts to images, adding easy user control to scene generation and editing by manipulating the input layout. This task known as semantic image synthesis spans many applications from data augmentation to model validation.  

%Graphics simulators have been traditionally used to generate synthetic data~\cite{gtav, carla}. While they allow the generation of diverse driving scenarios with realistic scene content, the generated images are not yet photorealistic, and they need expertise for the design and modeling of different urban scenes. Recently, learning-based graphics approaches, such as Generative Adversarial Networks (GANs) \cite{Goodfellow2014GenerativeAN}, have been proposed either to replace or to complement traditional approaches by enhancing their photorealism. Some initial approaches like image-to-image translation (I2I) \cite{epe, pix2pixhd, cyclegan} seek to translate synthetic images to photorealistic images, preserving their content but altering their texture. Although impressive results have been achieved~\cite{epe}, a drawback of this method is that it still depends on simulators for controllability. To edit a scene, one has to first use the graphics simulator for editing, then translate it to the real domain using the GAN model. On the other hand, semantic image synthesis (SIS) is a subclass of I2I where an image is generated from a semantic layout. SIS allows easy and explicit user control of scene editing through the manipulation of the input semantic map. For instance, one can add, delete or alter the style of different objects. SIS has been pivotal in several frameworks~\cite{palette, sbgan, decomposing} where semantic layouts are used as a prior for urban scene generation.

%Unsupervised approaches 


%Deep learning algorithms in autonomous driving need large amounts of annotated data for training and validation. A promise of synthetic data is to alleviate the extra costs associated with labeling, but it has to satisfy 2 properties for it to be really useful: photorealism and controllability. 

%In this work, we propose a practical paradigm to apply SIS in autonomous driving by exploiting cheaply available semantic layouts from a graphics simulator and real-life street-level images for the SIS task. We find that previous unpaired approaches underperform on this task because they operate on the assumption that source (labels) and target (images) domains share the same semantic distribution. As a remedy, we propose a novel framework, Syn2Real-USIS. Differently from previous works, which use only one discriminator overfitting the target domain statistics, we propose a framework with multiple discriminators operate on the image-level and multiscale patch-level. Moreover, to foster a stronger alignment with the input layout, we use the synthetic image as a guide to the generated image by minimizing the difference between their high-level attention features for a pre-trained VGG network. 

%While unpaired generative adversarial networks are suited for this task, they operate on the assumption that source (labels) and target (images) domains share the same semantic distribution. We find that previous approaches exhibit a performance drop on this task, as this assumption does not hold. 

%The need for large amounts of training and validation data is a huge concern in scaling AI algorithms for autonomous driving. A promise of generative adversarial networks (GANs) is to cut these costs by providing abundant photorealistic synthetic data. In particular, they can be used to translate semantic layouts to images of urban scenes, adding user control over scene generation and editing. However, conditional GANs used for label-to-image translation require paired data for training. In this work, we propose a practical solution to this issue: we leverage a set of synthetic labels from a graphics simulator and a set of street-level images recorded in real life for training an SIS model. While unsupervised frameworks can be leveraged for this task, they operate on the assumption that the source (labels) and target (images) share the same semantic distribution, which is untrue in this setting. We find that trained on two different distributions, unpaired frameworks exhibit a performance drop.    

  


%1-  In autonomous driving, label-to-image translation is highly desirable because it offers easy user control for urban scene generation and editing. Conditional Generative Adversarial Networks (cGANs) are used for this task to produce photorealistic images but need a large amount of expensive annotated data. A practical solution is to collect semantic layouts from a graphics simulator and to train an unpaired cGAN to translate between the synthetic layouts and real urban scenes. However, we find that state-of-the-art unpaired cGANs operate on the assumption that images and labels share the same semantic distribution, which is rarely the case in autonomous driving. As a result, we observe a performance drop. In this work, we make headway on this issue by designing a cross-domain GAN model for label-to-image translation. 


%2- Conditional Generative Adversarial Networks (cGANs) can translate semantic label maps to photorealistic images of urban scenes, which can be used for data augmentation. While unpaired cGANs can achieve this task and alleviate the need for expensive annotated images, they operate on the assumption that the unpaired images and labels share the same semantic distribution, which is rarely the case in practical scenarios. 

However, we find that the LPIPS loss can still leak information about the style and texture of $\xs$ into $\hat{x}^R$, which is undesirable (see Table \ref{tab:abl_disc}). Hypothesizing that this limitation comes from the nature of the convolutional $\mathrm{VGG}$ architectures (CNN), we turn towards vision transformers (ViT), which have recently shown a lot of success. Prior work on image classification has shown that CNNs tend to be biased towards texture~\cite{Geirhos2019ImageNettrainedCA}, while ViTs are more sensitive to object shapes, and more robust against domain shifts~\cite{daformer}, adversarial attacks, and color perturbations~\cite{intriguing, robustvit}. 

We examine the ViT architecture to identify which features can best encode the shape. In each transformer block, tokens from the previous layers ($F_{l-1}$) are projected through different linear layers with weights $W_Q, W_K, W_V$ into a query $Q$, key $K$ and value $V$ features, respectively. The similarity between $Q$ and $K$ is computed through a dot produced and normalized by the dimension of $K$, $d_K$, resulting in an $\mathrm{Attention}$ feature, which is then used as a weighted sum on $V$. The operations can be summarized as follows: 
{
 \begin{align}
 & Q = \mathrm{LN}(F_{l-1}) \cdot W_Q, \qquad K = \mathrm{LN}(F_{l-1}) \cdot W_K \nonumber\\
 &V = \mathrm{LN}(F_{l-1}) \cdot W_V \nonumber\\
 &\mathrm{Attention} = \frac{\mathrm{softmax}(Q \cdot K^T)}{\sqrt{d_K}}  \nonumber\\
 &F_{l}^{'} = \mathrm{Attention} \cdot V + F_{l-1} \nonumber\\
 &F_l = \mathrm{MLP}(\mathrm{LN}(F_l^{'})) + F_l^{'}          \nonumber
 \label{eq:transformer}
 \end{align}
}

We formulate the new transformer-based LPIPS loss function as a mean square error between the $\mathrm{Attention}$ features of $\xs$ and $\hat{x}^R$ extracted from the last layer ($M$) of a ViT pre-trained on ImageNet. We show later in Table \ref{tab:abl_vit} that the attention feature can encode the shape information more efficiently than other features inside the ViT (such as $K, F, Q$), because it is computed as the similarity between two sets of tokens in the high-dimensional feature space. Moreover, we choose to perform the alignment on the patch level, using the previously defined operator, $\mathcal{P}$, to achieve a more fine-grained alignment. The final loss can be expressed as:
{
 \begin{align}
& \mathcal{L}_{\mathrm{VIT-LPIPS}} = \left(\mathrm{Attention}_{M}(\mathcal{P}(\xs)) -\mathrm{Attention}_{M}(\mathcal{P}(\hat{x}^R)) \right)^2 \nonumber
 \end{align}
}

Our contributions in this part can be sumarized as: 
\begin{itemize}
    \item We use the last $\mathrm{Attention}$ feature of a pre-trained ViT to achieve alignment between $\xs$ and $\hat{x}^R$.
    \item We perform this alignment on the patch level as opposed to the image level, previously used in I2I frameworks \cite{spade, pix2pixhd}.
\end{itemize}

%The first setup is the ideal case, where the class distribution between images and labels is exactly the same. The second setup uses two datasets, as discussed in the problem formulation, and is the more realistic scenario. To test the models, we use the validation split of Cityscapes, which contains 500 annotated images for semantic segmentation. To measure the fidelity and alignment of generated images, we use the same metrics as previous supervised and unsupervised works~\cite{oasis, cut, usisicassp}. We report the FID and mIoU (alignment of the generated images with respect to the groundtruth labels) in Table \ref{table:study}. Results show that both models exhibit a considerable performance drop. 

%Measuring the performance on (1) is easy since the real datasets have paired data. In this case, we follow \cite{oasis, usisicassp} and measure the FID~\cite{heuselttur2017} and mean Intersection-over-Union (mIoU) of the generated images compared to the groundtruth labels. FID assesses both the diversity and quality of the generated images, while mIoU evaluates the quality and semantic alignment. For the second case, the synthetic labels only have corresponding synthetic images, which cannot be used as groundtruth. For this we follow the evaluation protocol of EPE~\cite{epe}, and measure the KVD. KVD computes the different between two sets of features, extracted from the generated images (which have synthetic layouts as input) and the images from the real dataset. Both sets are aligned, depending on the similarity of their semantic maps, as described in \cite{epe}. To summarize, for each benchmark, we report 3 metrics: FID and mIoU which are measured on the test splits of the real datasets, and KVD measured on the aligned synthetic and real sets. 
